Extending the Quantitative Pattern-Matching Paradigm

We show how (well-established) type systems based on non-idempotent intersection types can be extended to characterize termination properties of functional programming languages with pattern matching features. To model such programming languages, we use a (weak and closed) $\lambda$-calculus integrating a pattern matching mechanism on algebraic data types (ADTs). Remarkably, we also show that this language not only encodes Plotkin's CBV and CBN $\lambda$-calculus as well as other subsuming frameworks, such as the bang-calculus, but can also be used to interpret the semantics of effectful languages with exceptions. After a thorough study of the untyped language, we introduce a type system based on intersection types, and we show through purely logical methods that the set of terminating terms of the language corresponds exactly to that of well-typed terms. Moreover, by considering non-idempotent intersection types, this characterization turns out to be quantitative, i.e. the size of the type derivation of a term t gives an upper bound for the number of evaluation steps from t to its normal form.

==> proofs/confluence.tex <==
\begin{proof}
  Let us first prove that $\red{\HC}$ is \defn{subcommutative} (Def.1.1.8.(iv) of~\cite{Terese03}). Take any $t \in \calc$ such that $u \lred{\HC} t \red{\HC} r$. If $u = r$, then  we can immediately conclude. Otherwise, $u \neq  r$, and we can conclude by~\cref{lem:diamond}.

  It is well-known that subcommutativity implies confluence (Prop.1.1.10 of~\cite{Terese03}), so we can conclude that $\red{\HC}$ is confluent.
\end{proof}

==> proofs/no-one-step-loops.tex <==
\begin{proof}
    The proof follows by induction over $t \red{\HC} u$:
    \begin{itemize}
        \item Case $t = \MC \lhole{\lam p.r} s \onered[\ruleBeta] \MC \lhole{r \match{p}{s}} = u $, where $\bv{\MC} \cap \fv{s} = \eset$. We can conclude immediately.
        \item Case $t = \case{\MC \lhole{\ttc \vect{r_i}_n}}{(\ldots, \branch{\const{\ttc}{\vect{p_i}_n}}{s}, \ldots)} \onered[\ruleC] \MC \lhole{s \match{p_1}{r_1} \cdots \match{p_n}{r_n}} = u$, where $\bv{\MC} \cap \fv{s} = \eset$. We can conclude immediately.
        \item $t = r \match{\const{\ttc}{\vect{p_i}_n}}{\MC \lhole{\const{\ttc}{\vect{s_i}_n}}} \onered[\ruleM] \MC \lhole{r \match{p_1}{s_1} \cdots \match{p_n}{s_n}} = u$, where $\bv{\MC} \cap \fv{r} = \eset$. We can conclude immediately.
        \item Case $t = r \match{x}{s} \onered[\ruleE] r \subs{x}{s} = u$. Let us write $t = v \match{x_1}{s_1} \cdots \match{x_n}{s_n}$ in such a way that:
              \begin{itemize}
                  \item $n \geq 1$;
                  \item $x = x_n$ and $s = s_n$ (the last one);
                  \item and for all $1 \leq i \leq n$, $x_i \notin \fv{s_i} \cup \bv{s_i}$.
              \end{itemize}
              Consider $u = v \match{x_1}{s_1} \cdots \match{x_{n-1}}{s_{n-1}} \subs{x}{s} = v \subs{x}{s} \match{x_1}{s_1 \subs{x}{s}} \cdots \match{x_{n-1}}{s_{n-1} \subs{x}{s}}$. If $v \subs{x}{s}$ is not a closure, then $t$ has one more explicit substitution than $u$ at the top level, and thus we can conclude that $t \neq u$. If $v \subs{x}{s}$ is a closure, then it is necessarily the case that $v = x$, $s$ is a closure, and $t$ starts with a free occurrence of $x$, while $v \subs{x}{s} = s$ does not (by $\alpha$-conversion). Thus, we can conclude that $t \neq u$.
        \item The remaining cases follow easily from the \ih.
    \end{itemize}
\end{proof}
